Resilient Multi-Robot Target Tracking with Sensing and Communication Danger Zones

Multi-robot collaboration for target tracking in adversarial environments poses significant challenges, including system failures, dynamic priority shifts, and other unpredictable factors. These challenges become even more pronounced when the environment is unknown. In this paper, we propose a resilient coordination framework for multi-robot, multi-target tracking in environments with unknown sensing and communication danger zones. We consider scenarios where failures caused by these danger zones are probabilistic and temporary, allowing robots to escape from danger zones to minimize the risk of future failures. We formulate this problem as a nonlinear optimization with soft chance constraints, enabling real-time adjustments to robot behaviors based on varying types of dangers and failures. This approach dynamically balances target tracking performance and resilience, adapting to evolving sensing and communication conditions in real-time. To validate the effectiveness of the proposed method, we assess its performance across various tracking scenarios, benchmark it against methods without resilient adaptation and collaboration, and conduct several real-world experiments.

==> bib.tex <==
@inproceedings{bartolomei2020perception,
  title={Perception-aware path planning for uavs using semantic segmentation},
  author={Bartolomei, Luca and Teixeira, Lucas and Chli, Margarita},
  booktitle={2020 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
  pages={5808--5815},
  year={2020},
  organization={IEEE}
}


@article{wu2022perception,
  title={Perception-aware receding horizon trajectory planning for multicopters with visual-inertial odometry},
  author={Wu, Xiangyu and Chen, Shuxiao and Sreenath, Koushil and Mueller, Mark W},
  journal={IEEE Access},
  volume={10},
  pages={87911--87922},
  year={2022},
  publisher={IEEE}
}

@inproceedings{guo2019safe,
  title={Safe path planning with gaussian process regulated risk map},
  author={Guo, Hongliang and Meng, Zehui and Huang, Zefan and Kang, Leong Wei and Chen, Ziyue and Meghjani, Malika and Ang, Marcelo and Rus, Daniela},
  booktitle={2019 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)},
  pages={2044--2051},
  year={2019},
  organization={IEEE}
}

@article{zhou2011multirobot,
  title={Multirobot active target tracking with combinations of relative observations},
  author={Zhou, Ke and Roumeliotis, Stergios I},
  journal={IEEE Transactions on Robotics},
  volume={27},
  number={4},
  pages={678--695},
  year={2011},
  publisher={IEEE}
}

@inproceedings{schwager2017multi,
  title={A multi-robot control policy for information gathering in the presence of unknown hazards},
  author={Schwager, Mac and Dames, Philip and Rus, Daniela and Kumar, Vijay},
  booktitle={Robotics Research: The 15th International Symposium ISRR},
  pages={455--472},
  year={2017},
  organization={Springer}
}



